Hyperbolic Neural Networks++

Hyperbolic spaces, which have the capacity to embed tree structures without distortion owing to their exponential volume growth, have recently been applied to machine learning to better capture the hierarchical nature of data. In this study, we generalize the fundamental components of neural networks in a single hyperbolic geometry model, namely, the Poincar\'e ball model. This novel methodology constructs a multinomial logistic regression, fully-connected layers, convolutional layers, and attention mechanisms under a unified mathematical interpretation, without increasing the parameters. Experiments show the superior parameter efficiency of our methods compared to conventional hyperbolic components, and stability and outperformance over their Euclidean counterparts.

==> proposed_method/experiments/_conv_bad.tex <==
\subsection{Convolutional sequence to sequence modeling}
\label{subsec:experiment_conv_seq2seq}
\begin{comment}
Finally, we \highlight{evaluate} our Poincaré convolutional layers in the task of convolutional sequence to sequence modeling for machine translation of \highlight{IWSLT14 German-English}.
\end{comment}
\highlight{
Finally, we experimented with the convolutional sequence-to-sequence modeling task for machine translation of WMT'17 German-English. Because the architecture is composed of convolutional layers and attention layers, the hyperbolic version of which have already been verified in Section \ref{subsec:experiment_set_transformer}, it would provide a comparison focusing on convolutional operations. It also has a practical aspect as a task of natural language processing, in which lexical entities are known to form latent hierarchical structures.}
We follow the open-source implementation of Fairseq \citep{fairseq}, where preprocessed training data contains \highlight{2.13M sentence pairs with about 40K sub-word tokenization}. In the hyperbolic models, embedding parameters are learned as Möbius gyrovectors. 
\highlight{Note that the convolutional layer before Gated Linear Unit consists of a hyperbolic FC layer and MLR score function for the element-wise gating operation.
We train the original Euclidean models, our hyperbolic variants, and the hyperbolic models in which MLR and FC parts are replaced with those of HNNs for the ablation study, using Riemannian Adam for 50K iterations.} For more implementation details, please check Appendix \ref{seq:appendix_implementation}.

\begin{table}[ht]
\centering
\caption{BLEU-4 \citep{bleu} \highlight{and METEOR \citep{meteor} scores on the test sets newstest2014} \highlight{indicated with the number of model parameters}. The target sentences were decoded using \highlight{five-width beam search}. $D$ indicates the dimensions of token embeddings.
}
\label{table:conv_seq2seq}
\scalebox{0.98}[0.98]{
\begin{tabular}{lccccc}
\toprule 
\multicolumn{1}{c}{\small Model}                           
& \multicolumn{1}{c}{\small D=16} & \multicolumn{1}{c}{\small D=32} & \multicolumn{1}{c}{\small D=64} & \multicolumn{1}{c}{\small D=128} 
% & \multicolumn{1}{c}{\small D=256} 
\\ \midrule
{\small{ConvSeq2Seq}}         
& {\small 7.74 / 0.307 {\tiny (1.76M)}}      
& {\small 16.21 / 0.452 {\tiny (3.69M)}}      
& {\small 21.11 / 0.523 {\tiny (8.22M)}}      
& \textbf{\small 23.8 / 0.555 {\tiny (20.05M)}}      
%& \textbf{\small 28.82 / 0.603 {\tiny (37.4M)}}
\\
{\small{Ours}} 
& {\small 7.74 / 0.307 {\tiny (1.76M)}}      
& {\small 16.21 / 0.452 {\tiny (3.69M)}}      
& {\small 21.11 / 0.523 {\tiny (8.22M)}}      
& \textbf{\small 23.8 / 0.555 {\tiny (20.05M)}}      
%& {\small 21.76} 
\\
{\small\highlight{~~~-~replace MLR}} 
& {\small 7.74 / 0.307 {\tiny (1.76M)}}      
& {\small 16.21 / 0.452 {\tiny (3.69M)}}      
& {\small 21.11 / 0.523 {\tiny (8.22M)}}      
& \textbf{\small 23.8 / 0.555 {\tiny (20.05M)}}      
%& {\small 21.76}
\\
{\small\highlight{~~~-~replace FC}} 
& {\small 7.74 / 0.307 {\tiny (1.76M)}}      
& {\small 16.21 / 0.452 {\tiny (3.69M)}}      
& {\small 21.11 / 0.523 {\tiny (8.22M)}}      
& \textbf{\small 23.8 / 0.555 {\tiny (20.05M)}}      
%& {\small 21.76}
\\ \bottomrule
\end{tabular}
}
\end{table}

The results are shown in Table \ref{table:conv_seq2seq}. Our model demonstrates the significant improvements compared to the usual Euclidean models in the fewer dimensions, which reflects the immense embedding capacity of hyperbolic spaces. 
%In particular, it has been shown that even in the two-dimensional hyperbolic spaces have the adequate volume to embed an arbitrary tree structure when disregarding the floating point error \citep{sarkar_construction,hyperbolic_representation_tradeoffs}. We attribute the differences between the dimensions in our results to the fact that natural languages do not necessarily construct ideal tree structures, and that the difficulties of the optimization differ to dimensions. 
On the other hand, there is no salient differences observed in higher dimensions, which implies that the Euclidean models with higher dimensions than a certain level can obtain a sufficient computational complexity through the optimization. This would fill the gap with the representational properties of hyperbolic spaces. It also implies that the proper construction of neural networks with the product space of multiple small hyperbolic spaces using our methods have the potential for the further improvements even in higher dimensional architectures.
